Efficient inference of overlapping communities in complex networks

We discuss two views on extending existing methods for complex network modeling which we dub the communities first and the networks first view, respectively. Inspired by the networks first view that we attribute to White, Boorman, and Breiger (1976)[1], we formulate the multiple-networks stochastic blockmodel (MNSBM), which seeks to separate the observed network into subnetworks of different types and where the problem of inferring structure in each subnetwork becomes easier. We show how this model is specified in a generative Bayesian framework where parameters can be inferred efficiently using Gibbs sampling. The result is an effective multiple-membership model without the drawbacks of introducing complex definitions of "groups" and how they interact. We demonstrate results on the recovery of planted structure in synthetic networks and show very encouraging results on link prediction performances using multiple-networks models on a number of real-world network data sets.

==> ex-disjoint-sbm.tex <==
\begin{tikzpicture}[node distance=1.2cm,bend angle=30,auto]
	
	% Psoudo-node for vertical alignment
	\begin{scope}[yshift=-3.1cm]
		\node [place, opacity=0] (psn1) [] {};
	\end{scope}
	
	\node [place] (sn1) {1};
	\node [place] (sn2) [below of=sn1] {2}
		edge node[inner sep=1pt] {5} (sn1);
	\node [place] (sn3) [right of=sn1, yshift=-6mm] {3}
		edge node[inner sep=1pt,swap] {4} (sn1)
		edge node[inner sep=1pt] {4} (sn2);
		
	\node [place] (sn4) [right of=sn3,xshift=5mm] {4}
		edge node[inner sep=1pt] {6} (sn3)
		edge [bend right] node[inner sep=1pt] {4} (sn1)
		edge [bend left] node[inner sep=1pt,swap] {4} (sn2);
	\node [place] (sn5) [right of=sn4, yshift=6mm] {5}
		edge node[inner sep=1pt,swap] {2} (sn4)
		edge [bend right] node[inner sep=1pt] {2} (sn3);
	\node [place] (sn6) [below of=sn5] {6}
		edge node[inner sep=1pt,swap] {4} (sn5)
		edge node[inner sep=1pt] {2} (sn4)
		edge [bend left] node[inner sep=1pt,swap] {2} (sn3);
		
	\begin{scope}[yshift=-.47cm,xshift=5.7cm]
		\node (eta1){ %
			\footnotesize
			\begin{minipage}{0cm}
			\begin{align*}
			\m \eta &= 
			\begin{vmatrix}
			5 & & & \\
			4 & 4 & & \\
			4 & 6 & 2 & \\
			0 & 2 & 2  & 4\\
			\end{vmatrix}
			\end{align*}
			\end{minipage}	
		};
	\end{scope}
	
	\begin{pgfonlayer}{background}
	
%		\tikzset{cluster/.style={rectangle, inner sep=1mm, rounded corners=2mm}};
		
		% Color single network clusters
		\node [cluster, fill=blue!30,
		fit=(sn1) (sn2)] {};
		\node [cluster, fill=yellow!50,
		fit=(sn3)] {};
		\node [cluster, fill=red!30,
		fit=(sn4)] {};
		\node [cluster, fill=green!30,
		fit=(sn5) (sn6)] {};
		% End color single network clusters
		
	\end{pgfonlayer}
		
		
\end{tikzpicture}

==> ex-mnsbm.tex <==
\begin{tikzpicture}[node distance=1.2cm,bend angle=30,auto]
	
	\begin{scope}
		\node [place] (s1n1) {1};
		\node [place] (s1n2) [below of=s1n1] {2}
			edge node[inner sep=1pt] {4} (s1n1);
		\node [place] (s1n3) [right of=s1n1, yshift=-6mm] {3}
			edge node[inner sep=1pt,swap] {4} (s1n1)
			edge node[inner sep=1pt] {4} (s1n2);
	
		\node [place] (s1n4) [right of=s1n3,xshift=5mm] {4}
			edge node[inner sep=1pt] {4} (s1n3)
			edge [bend right] node[inner sep=1pt] {4} (s1n1)
			edge [bend left] node[inner sep=1pt,swap] {4} (s1n2);
		\node [place] (s1n5) [right of=s1n4, yshift=6mm] {5};
		\node [place] (s1n6) [below of=s1n5] {6}
			edge node[inner sep=1pt,swap] {2} (s1n5);
	\end{scope}
	
	\begin{scope}[yshift=-0.47cm,xshift=5.7cm]
		\node (eta1){ %
			\footnotesize
			\begin{minipage}{0cm}
			\begin{align*}
			\m \eta_1 &= 
			\begin{vmatrix}
			4 & \\
			0 & 2 \\
			\end{vmatrix}
			\end{align*}
			\end{minipage}	
		};
	\end{scope}
	
	\begin{scope}[yshift=-3cm]
		\node [place] (s2n1) {1};
		\node [place] (s2n2) [below of=s2n1] {2}
			edge node[inner sep=1pt] {1} (s2n1);
		\node [place] (s2n3) [right of=s2n1, yshift=-6mm] {3};
		
		\node [place] (s2n4) [right of=s2n3,xshift=5mm] {4}
			edge node[inner sep=1pt] {2} (s2n3);
		\node [place] (s2n5) [right of=s2n4, yshift=6mm] {5}
			edge node[inner sep=1pt,swap] {2} (s2n4)
			edge [bend right] node[inner sep=1pt] {2} (s2n3);
		\node [place] (s2n6) [below of=s2n5] {6}
			edge node[inner sep=1pt,swap] {2} (s2n5)
			edge node[inner sep=1pt] {2} (s2n4)
			edge [bend left] node[inner sep=1pt,swap] {2} (s2n3);
	\end{scope}
	
	\begin{scope}[yshift=-3.47cm,xshift=5.7cm]
		\node (eta1){ %
			\footnotesize
			\begin{minipage}{0cm}
			\begin{align*}
			\m \eta_2 &= 
			\begin{vmatrix}
			1 & \\
			0 & 2 \\
			\end{vmatrix}
			\end{align*}
			\end{minipage}	
		};
	\end{scope}
	
	\begin{pgfonlayer}{background}
	
%		\tikzset{cluster/.style={rectangle, inner sep=1mm, rounded corners=2mm}};
		
		% Color subnetwork clusters
		\node [cluster, fill=blue!30,
			fit=(s1n1) (s1n2) (s1n4)] {};
		\node [cluster, fill=green!30,
			fit=(s1n5) (s1n6)] {};
		\node [cluster, fill=yellow!50,
			fit=(s2n1) (s2n2)] {};
		\node [cluster, fill=red!30,
			fit=(s2n3) (s2n5) (s2n6)] {};
		% End color subnetwork clusters
		
%		\tikzset{black dashed/.style={
%			draw=black!50!white, dashed, line width=1pt,
%			inner sep=3mm, rounded corners
%		}};
		
		% Draw dashed boxes with labels around subnetworks
		\node (subnetwork1) [black dashed,
			fit =(s1n1) (s1n2) (s1n5)] {};
		\node at (subnetwork1.north) [above, inner sep=1mm] {Subnetwork 1};
		\node (subnetwork2) [black dashed,
			fit =(s2n1) (s2n2) (s2n5)] {};
		\node at (subnetwork2.north) [above, inner sep=1mm] {Subnetwork 2};
		% End dashed boxes

	\end{pgfonlayer}
	
\end{tikzpicture}

==> ex-obs-network.tex <==
\begin{tikzpicture}[node distance=1.2cm,bend angle=30,auto]
	
	% Psoudo-node for vertical alignment
	\begin{scope}[yshift=-3.1cm]
		\node [place, opacity=0] (psn1) [] {};
	\end{scope}
	
	\node [place] (n1) {1};
	\node [place] (n2) [below of=n1] {2}
		edge node[inner sep=1pt] {5} (n1);
	\node [place] (n3) [right of=n1, yshift=-6mm] {3}
		edge node[inner sep=1pt,swap] {4} (n1)
		edge node[inner sep=1pt] {4} (n2);
	
	\node [place] (n4) [right of=n3,xshift=5mm] {4}
		edge node[inner sep=1pt] {6} (n3)
		edge [bend right] node[inner sep=1pt] {4} (n1)
		edge [bend left] node[inner sep=1pt,swap] {4} (n2);
	\node [place] (n5) [right of=n4, yshift=6mm] {5}
		edge node[inner sep=1pt,swap] {2} (n4)
		edge [bend right] node[inner sep=1pt] {2} (n3);
	\node [place] (n6) [below of=n5] {6}
		edge node[inner sep=1pt,swap] {4} (n5)
		edge node[inner sep=1pt] {2} (n4)
		edge [bend left] node[inner sep=1pt,swap] {2} (n3);
\end{tikzpicture}

==> figures/tikz/ex-networks/ex-disjoint-sbm.tex <==
\begin{tikzpicture}[node distance=1.2cm,bend angle=30,auto]
	
	% Psoudo-node for vertical alignment
	\begin{scope}[yshift=-3.1cm]
		\node [place, opacity=0] (psn1) [] {};
	\end{scope}
	
	\node [place] (sn1) {1};
	\node [place] (sn2) [below of=sn1] {2}
		edge node[inner sep=1pt] {5} (sn1);
	\node [place] (sn3) [right of=sn1, yshift=-6mm] {3}
		edge node[inner sep=1pt,swap] {4} (sn1)
		edge node[inner sep=1pt] {4} (sn2);
		
	\node [place] (sn4) [right of=sn3,xshift=5mm] {4}
		edge node[inner sep=1pt] {6} (sn3)
		edge [bend right] node[inner sep=1pt] {4} (sn1)
		edge [bend left] node[inner sep=1pt,swap] {4} (sn2);
	\node [place] (sn5) [right of=sn4, yshift=6mm] {5}
		edge node[inner sep=1pt,swap] {2} (sn4)
		edge [bend right] node[inner sep=1pt] {2} (sn3);
	\node [place] (sn6) [below of=sn5] {6}
		edge node[inner sep=1pt,swap] {4} (sn5)
		edge node[inner sep=1pt] {2} (sn4)
		edge [bend left] node[inner sep=1pt,swap] {2} (sn3);
		
	\begin{scope}[yshift=-.47cm,xshift=5.7cm]
		\node (eta1){ %
			\footnotesize
			\begin{minipage}{0cm}
			\begin{align*}
			\m \eta &= 
			\begin{vmatrix}
			5 & & & \\
			4 & 4 & & \\
			4 & 6 & 2 & \\
			0 & 2 & 2  & 4\\
			\end{vmatrix}
			\end{align*}
			\end{minipage}	
		};
	\end{scope}
	
	\begin{pgfonlayer}{background}
	
%		\tikzset{cluster/.style={rectangle, inner sep=1mm, rounded corners=2mm}};
		
		% Color single network clusters
		\node [cluster, fill=blue!30,
		fit=(sn1) (sn2)] {};
		\node [cluster, fill=yellow!50,
		fit=(sn3)] {};
		\node [cluster, fill=red!30,
		fit=(sn4)] {};
		\node [cluster, fill=green!30,
		fit=(sn5) (sn6)] {};
		% End color single network clusters
		
	\end{pgfonlayer}
		
		
\end{tikzpicture}

==> figures/tikz/ex-networks/ex-mnsbm.tex <==
\begin{tikzpicture}[node distance=1.2cm,bend angle=30,auto]
	
	\begin{scope}
		\node [place] (s1n1) {1};
		\node [place] (s1n2) [below of=s1n1] {2}
			edge node[inner sep=1pt] {4} (s1n1);
		\node [place] (s1n3) [right of=s1n1, yshift=-6mm] {3}
			edge node[inner sep=1pt,swap] {4} (s1n1)
			edge node[inner sep=1pt] {4} (s1n2);
	
		\node [place] (s1n4) [right of=s1n3,xshift=5mm] {4}
			edge node[inner sep=1pt] {4} (s1n3)
			edge [bend right] node[inner sep=1pt] {4} (s1n1)
			edge [bend left] node[inner sep=1pt,swap] {4} (s1n2);
		\node [place] (s1n5) [right of=s1n4, yshift=6mm] {5};
		\node [place] (s1n6) [below of=s1n5] {6}
			edge node[inner sep=1pt,swap] {2} (s1n5);
	\end{scope}
	
	\begin{scope}[yshift=-0.47cm,xshift=5.4cm]
		\node (eta1){ %
			\footnotesize
			\begin{minipage}{0cm}
			\begin{align*}
			\m \eta_1 &= 
			\begin{vmatrix}
			4 & \\
			0 & 2 \\
			\end{vmatrix}
			\end{align*}
			\end{minipage}	
		};
	\end{scope}
	
	\begin{scope}[yshift=-3cm]
		\node [place] (s2n1) {1};
		\node [place] (s2n2) [below of=s2n1] {2}
			edge node[inner sep=1pt] {1} (s2n1);
		\node [place] (s2n3) [right of=s2n1, yshift=-6mm] {3};
		
		\node [place] (s2n4) [right of=s2n3,xshift=5mm] {4}
			edge node[inner sep=1pt] {2} (s2n3);
		\node [place] (s2n5) [right of=s2n4, yshift=6mm] {5}
			edge node[inner sep=1pt,swap] {2} (s2n4)
			edge [bend right] node[inner sep=1pt] {2} (s2n3);
		\node [place] (s2n6) [below of=s2n5] {6}
			edge node[inner sep=1pt,swap] {2} (s2n5)
			edge node[inner sep=1pt] {2} (s2n4)
			edge [bend left] node[inner sep=1pt,swap] {2} (s2n3);
	\end{scope}
	
	\begin{scope}[yshift=-3.47cm,xshift=5.4cm]
		\node (eta2){ %
			\footnotesize
			\begin{minipage}{0cm}
			\begin{align*}
			\m \eta_2 &= 
			\begin{vmatrix}
			1 & \\
			0 & 2 \\
			\end{vmatrix}
			\end{align*}
			\end{minipage}	
		};
	\end{scope}
	
	\begin{pgfonlayer}{background}
	
%		\tikzset{cluster/.style={rectangle, inner sep=1mm, rounded corners=2mm}};
		
		% Color subnetwork clusters
		\node [cluster, fill=blue!30,
			fit=(s1n1) (s1n2) (s1n4)] {};
		\node [cluster, fill=green!30,
			fit=(s1n5) (s1n6)] {};
		\node [cluster, fill=yellow!50,
			fit=(s2n1) (s2n2)] {};
		\node [cluster, fill=red!30,
			fit=(s2n3) (s2n5) (s2n6)] {};
		% End color subnetwork clusters
		
%		\tikzset{black dashed/.style={
%			draw=black!50!white, dashed, line width=1pt,
%			inner sep=3mm, rounded corners
%		}};
		
		% Draw dashed boxes with labels around subnetworks
		\node (subnetwork1) [black dashed,
			fit =(s1n1) (s1n2) (s1n5) (eta1)] {};
		\node at (subnetwork1.north) [above, inner sep=1mm] {Subnetwork 1};
		\node (subnetwork2) [black dashed,
			fit =(s2n1) (s2n2) (s2n5) (eta2)] {};
		\node at (subnetwork2.north) [above, inner sep=1mm] {Subnetwork 2};
		% End dashed boxes

	\end{pgfonlayer}
	
\end{tikzpicture}

==> figures/tikz/ex-networks/ex-obs-network.tex <==
\begin{tikzpicture}[node distance=1.2cm,bend angle=30,auto]
	
	% Psoudo-node for vertical alignment
	\begin{scope}[yshift=-3.1cm]
		\node [place, opacity=0] (psn1) [] {};
	\end{scope}
	
	\node [place] (n1) {1};
	\node [place] (n2) [below of=n1] {2}
		edge node[inner sep=1pt] {5} (n1);
	\node [place] (n3) [right of=n1, yshift=-6mm] {3}
		edge node[inner sep=1pt,swap] {4} (n1)
		edge node[inner sep=1pt] {4} (n2);
	
	\node [place] (n4) [right of=n3,xshift=5mm] {4}
		edge node[inner sep=1pt] {6} (n3)
		edge [bend right] node[inner sep=1pt] {4} (n1)
		edge [bend left] node[inner sep=1pt,swap] {4} (n2);
	\node [place] (n5) [right of=n4, yshift=6mm] {5}
		edge node[inner sep=1pt,swap] {2} (n4)
		edge [bend right] node[inner sep=1pt] {2} (n3);
	\node [place] (n6) [below of=n5] {6}
		edge node[inner sep=1pt,swap] {4} (n5)
		edge node[inner sep=1pt] {2} (n4)
		edge [bend left] node[inner sep=1pt,swap] {2} (n3);
\end{tikzpicture}
